Constant-Cost Spatio-Angular Prefiltering of Glinty Appearance Using Tensor Decomposition

The detailed glinty appearance from complex surface microstructures enhances the level of realism, but is both space- and time-consuming to render, especially when viewed from far away (large spatial coverage) and/or illuminated by area lights (large angular coverage). In this paper, we formulate the glinty appearance rendering process as a spatio-angular range query problem of the Normal Distribution Functions (NDFs), and introduce an efficient spatio-angular prefiltering solution to it. We start by exhaustively precomputing all possible NDFs with differently sized positional coverages. Then we compress the precomputed data using tensor rank decomposition, which enables accurate and fast angular range queries. With our spatio-angular prefiltering scheme, we are able to solve both the storage and performance issues at the same time, leading to efficient rendering of glinty appearance with both constant storage and constant performance, regardless of the range of spatio-angular queries. Finally, we demonstrate that our method easily applies to practical rendering applications that were traditionally considered difficult. For example, efficient bidirectional reflection distribution function (BRDF) evaluation accurate NDF importance sampling, fast global illumination between glinty objects, high-frequency preserving rendering with environment lighting, and tile-based synthesis of glinty appearance.

==> paper_NewTable.tex <==
 \begin{table*}[htbp]
  \caption{\label{tab:}The precomputation cost of each texture. Texture is the normal map we used for geometric optics. If we use wave optics, it means a heightfield map. Type is geometric or wave. Res. is the resolution of the texture.{Traversal means path cut hierarchical pruning until a path consisting of leaf nodes, Newton solving means solving for specular light paths with Newton solver, and splatting means projecting the specular light paths to the screen space and computing the pixel radiance. \#Glint is the glint count.}} 
\centering
\begin{tabular}{lccccccccccl}
\toprule
   \multicolumn{1}{c}{Texture}
	 & \multicolumn{1}{c}{Type}
	 & \multicolumn{1}{c}{Res.}
	 & \multicolumn{1}{c}{Generate time(min.)}
	 & \multicolumn{1}{c}{Compression time(min.)}
	 & \multicolumn{1}{c}{Total Time (min.)}
	 & \multicolumn{1}{c}{Storage cost (MB)} \\	
		%\midrule
		Deer         &{Fig. 5}  & 9210.5 & Metal        & RR & 4.51   & 1.86   & 0.07  & 6.44  & 1000.87& 12902 \\ \hline 
		Single Slab  &{Fig. 12} 	& 500    & Metal        & R  & 0.16   & 0.05   & 0.034  & 0.24   & 56.47 & 5135 \\ \hline 
		Double Slab  &{Fig. 6}	& 1000   & Glass (1.50) & TT  & 1.00  & 0.32   & 0.095  & 1.42   & 112.94 & 16323\\ \hline 
		Double Slab  &{Fig. 8} 	& 1000   & Glass (1.50) & TRT & 5.46  & 6.42   & 0.072  & 11.95  & 112.94 & 9454 \\ \hline 
	 	Double Slab  &{Fig. 10} 	& 2000   & Glass (1.50) & TTTT& 42.76 & 51.65  & 0.014  & 94.42  & 225.87 & 721 \\ \hline 
		Splash 	     &{Fig. 1}  & 49.8   & Water (1.33) & TT  & 6.36  & 1.13   & 0.008  & 7.50   & 4.64   & 174 \\ \hline 
		Splash       &{Fig. 1}  &49.8    &Water(1.33)   &TRT  &135.32 & 345.35 & 0.009  &480.68  & 4.64   &212\\\hline 
		Stained Glass&{Fig. 9}  & 205.5  & Glass (1.50) & TT & 30.28 & 22.73 & 0.018  & 53.03 & 20.84  & 3502 \\ 
\bottomrule

\end{tabular}
\end{table*}




==> paper_scene.tex <==
 \begin{table*}[htbp]
  \caption{\label{tab:}Scene settings, computation time and memory costs for our test scenes. \#Tri. is the count of triangles in the scene. Type means the type of light transport, such as Reflection-Reflection, Transmittance-Transmittance, or Transmittance-Reflection-Transmittance. {Traversal means path cut hierarchical pruning until a path consisting of leaf nodes, Newton solving means solving for specular light paths with Newton solver, and splatting means projecting the specular light paths to the screen space and computing the pixel radiance. \#Glint is the glint count.}} 
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccl}
\toprule
   \multicolumn{1}{c}{Scene}
	 & \multicolumn{1}{c}{Fig.}
	 & \multicolumn{1}{c}{\#Tri.(K)}
	 & \multicolumn{1}{c}{Material.}
	 & \multicolumn{1}{c}{Type}
	 & \multicolumn{4}{c}{Time (sec.)}
	 & \multicolumn{1}{c}{Memory (MB)}
	 & \multicolumn{1}{c}{\#Glint} \\	
  \cmidrule(lr){6-9}
	               &        &        &              &    & Traversal & Newton solving & Splatting & Total & & \\
		\midrule
		Deer         &{Fig. 5}  & 9210.5 & Metal        & RR & 4.51   & 1.86   & 0.07  & 6.44  & 1000.87& 12902 \\ \hline 
		Single Slab  &{Fig. 12} 	& 500    & Metal        & R  & 0.16   & 0.05   & 0.034  & 0.24   & 56.47 & 5135 \\ \hline 
		Double Slab  &{Fig. 6}	& 1000   & Glass (1.50) & TT  & 1.00  & 0.32   & 0.095  & 1.42   & 112.94 & 16323\\ \hline 
		Double Slab  &{Fig. 8} 	& 1000   & Glass (1.50) & TRT & 5.46  & 6.42   & 0.072  & 11.95  & 112.94 & 9454 \\ \hline 
	 	Double Slab  &{Fig. 10} 	& 2000   & Glass (1.50) & TTTT& 42.76 & 51.65  & 0.014  & 94.42  & 225.87 & 721 \\ \hline 
		Splash 	     &{Fig. 1}  & 49.8   & Water (1.33) & TT  & 6.36  & 1.13   & 0.008  & 7.50   & 4.64   & 174 \\ \hline 
		Splash       &{Fig. 1}  &49.8    &Water(1.33)   &TRT  &135.32 & 345.35 & 0.009  &480.68  & 4.64   &212\\\hline 
		Stained Glass&{Fig. 9}  & 205.5  & Glass (1.50) & TT & 30.28 & 22.73 & 0.018  & 53.03 & 20.84  & 3502 \\ 
\bottomrule

\end{tabular}
}
\end{table*}



